Automated Refactoring of Nested-IF Formulae in Spreadsheets

Spreadsheets are the most popular end-user programming software, where formulae act like programs and also have smells. One well recognized common smell of spreadsheet formulae is nest-IF expressions, which have low readability and high cognitive cost for users, and are error-prone during reuse or maintenance. However, end users usually lack essential programming language knowledge and skills to tackle or even realize the problem. The previous research work has made very initial attempts in this aspect, while no effective and automated approach is currently available. This paper firstly proposes an AST-based automated approach to systematically refactoring nest-IF formulae. The general idea is two-fold. First, we detect and remove logic redundancy on the AST. Second, we identify higher-level semantics that have been fragmented and scattered, and reassemble the syntax using concise built-in functions. A comprehensive evaluation has been conducted against a real-world spreadsheet corpus, which is collected in a leading IT company for research purpose. The results with over 68,000 spreadsheets with 27 million nest-IF formulae reveal that our approach is able to relieve the smell of over 99\% of nest-IF formulae. Over 50% of the refactorings have reduced nesting levels of the nest-IFs by more than a half. In addition, a survey involving 49 participants indicates that for most cases the participants prefer the refactored formulae, and agree on that such automated refactoring approach is necessary and helpful.

==> Makefile <==
# makefile for pdf2latex
name=bare_conf

#open: allfontpdf
open: pdf
		open -a Preview ${name}.pdf;
pdf:
		pdflatex ${name}; 
		pdflatex ${name}.tex; 
		bibtex ${name}
		pdflatex ${name}.tex; 
allfontpdf:
	bibtex ${name}
	latex ${name}.tex
	dvips ${name}
	bibtex ${name}
	ps2pdf -dSubsetFonts=true -dEmbedAllFonts=true -dCompatibilityLevel=1.4 -dPDFSETTINGS=/prepress -sPAPERSIZE=letter ${name}.ps ${name}.pdf
clean: 
	rm -rf ${name}.aux ${name}.bbl ${name}.log ${name}.blg\
	 ${name}.out ${name}.out.bak ${name}.ps ${name}.dvi *~


==> macros.tex <==
%\usepackage{times}
%\usepackage{graphicx}
%\usepackage{epsf}
%\usepackage{verbatim}
%\usepackage{psfig}
%\usepackage{cite}
\usepackage{url}
\usepackage{color}
\usepackage{alltt}

\newcommand{\Framework}{}


\newcommand{\Add}{\CodeIn{add}}
\newcommand{\AVTree}{\CodeIn{AVTree}}
\newcommand{\Assignment}[3]{$\langle$ \Object{#1}, \Object{#2}, \Object{#3} $\rangle$}
\newcommand{\BinaryTreeRemove}{\CodeIn{BinaryTree\_remove}}
\newcommand{\BinaryTree}{\CodeIn{BinaryTree}}
\newcommand{\Caption}{\caption}
\newcommand{\Char}[1]{`#1'}
\newcommand{\CheckRep}{\CodeIn{checkRep}}
\newcommand{\ClassC}{\CodeIn{C}}
\newcommand{\CodeIn}[1]{{\small\texttt{#1}}}
\newcommand{\CodeOutSize}{\scriptsize}
\newcommand{\Comment}[1]{}
\newcommand{\Ensures}{\CodeIn{ensures}}
\newcommand{\ExtractMax}{\CodeIn{extractMax}}
\newcommand{\FAL}{field-ordering}
\newcommand{\FALs}{field-orderings}
\newcommand{\Fact}{observation}
\newcommand{\Get}{\CodeIn{get}}
\newcommand{\HashSet}{\CodeIn{HashSet}}
\newcommand{\HeapArray}{\CodeIn{HeapArray}}
\newcommand{\Intro}[1]{\emph{#1}}
\newcommand{\Invariant}{\CodeIn{invariant}}
\newcommand{\JUC}{\CodeIn{java.\-util.\-Collections}}
\newcommand{\JUS}{\CodeIn{java.\-util.\-Set}}
\newcommand{\JUTM}{\CodeIn{java.\-util.\-TreeMap}}
\newcommand{\JUTS}{\CodeIn{java.\-util.\-TreeSet}}
\newcommand{\JUV}{\CodeIn{java.\-util.\-Vector}}
\newcommand{\JMLPlusJUnit}{JML+JUnit}
\newcommand{\Korat}{Korat}
\newcommand{\Left}{\CodeIn{left}}
\newcommand{\Lookup}{\CodeIn{lookup}}
\newcommand{\MethM}{\CodeIn{m}}
\newcommand{\Node}[1]{\CodeIn{N}$_#1$}
\newcommand{\Null}{\CodeIn{null}}
\newcommand{\Object}[1]{\CodeIn{o}\ensuremath{_#1}}
\newcommand{\PostM}{\MethM$_{post}$}
\newcommand{\PreM}{\MethM$_{pre}$}
\newcommand{\Put}{\CodeIn{put}}
\newcommand{\Remove}{\CodeIn{remove}}
\newcommand{\RepOk}{\CodeIn{repOk}}
\newcommand{\Requires}{\CodeIn{requires}}
\newcommand{\Reverse}{\CodeIn{reverse}}
\newcommand{\Right}{\CodeIn{right}}
\newcommand{\Root}{\CodeIn{root}}
\newcommand{\Set}{\CodeIn{set}}
\newcommand{\State}[1]{2^{#1}}
\newcommand{\TestEra}{TestEra}
\newcommand{\TreeMap}{\CodeIn{TreeMap}}

\newenvironment{CodeOut}{\begin{scriptsize}}{\end{scriptsize}}
\newenvironment{SmallOut}{\begin{small}}{\end{small}}

\newcommand{\pairwiseEquals}{PairwiseEquals}
\newcommand{\monitorEquals}{MonitorEquals}
%\newcommand{\monitorWField}{WholeStateW}
\newcommand{\traverseField}{WholeState}
\newcommand{\monitorSMSeq}{ModifyingSeq}
\newcommand{\monitorSeq}{WholeSeq}

\newcommand{\IntStack}{\CodeIn{IntStack}}
\newcommand{\UBStack}{\CodeIn{UBStack}}
\newcommand{\BSet}{\CodeIn{BSet}}
\newcommand{\BBag}{\CodeIn{BBag}}
\newcommand{\ShoppingCart}{\CodeIn{ShoppingCart}}
\newcommand{\BankAccount}{\CodeIn{BankAccount}}
\newcommand{\BinarySearchTree}{\CodeIn{BinarySearchTree}}
\newcommand{\LinkedList}{\CodeIn{LinkedList}}

\newcommand{\Book}{\CodeIn{Book}}
\newcommand{\Library}{\CodeIn{Library}}

\newcommand{\Jtest}{Jtest}
\newcommand{\JCrasher}{JCrasher}
\newcommand{\Daikon}{Daikon}
\newcommand{\JUnit}{JUnit}

\newcommand{\trie}{trie}

\newcommand{\Perl}{Perl}


\newcommand{\SubjectCount}{11}
\newcommand{\DSSubjectCount}{two}

\newcommand{\Equals}{\CodeIn{equals}}
\newcommand{\Pairwise}{PairwiseEquals}
\newcommand{\Subgraph}{MonitorEquals}
\newcommand{\Concrete}{WholeState}
\newcommand{\ModSeq}{ModifyingSeq}
\newcommand{\Seq}{WholeSeq}
\newcommand{\Aeq}{equality}

\newcommand{\Meaning}[1]{\ensuremath{[\![}#1\ensuremath{]\!]}}
\newcommand{\Pair}[2]{\ensuremath{\langle #1, #2 \rangle}}
\newcommand{\Triple}[3]{\ensuremath{\langle #1, #2, #3 \rangle}}
\newcommand{\SetSuch}[2]{\ensuremath{\{ #1 | #2 \}}}
%\newtheorem{definition}{Definition}
%\newtheorem{theorem}[definition]{Theorem}
\newcommand{\Equiv}[2]{\ensuremath{#1 \EquivSTRel{} #2}}
\newcommand{\EquivME}{\Equiv}
\newcommand{\EquivST}{\Equiv}
\newcommand{\EquivSTRel}{\ensuremath{\cong}}
\newcommand{\Redundant}[2]{\ensuremath{#1 \lhd #2}}
\newcommand{\VB}{\ensuremath{\mid}}
\newcommand{\MES}{method-entry state}

%\newcommand{\Small}[1]{{\small{#1}}}

\newcommand{\CenterCell}[1]{\multicolumn{1}{c|}{#1}}


\newcommand{\pure}{\CodeIn{pure}}
\newcommand{\correct}{\CodeIn{correct}}
\newcommand{\visitor}{\CodeIn{Visitor}}
\newcommand{\savethis}{\CodeIn{savethis}}

\newcommand{\SLOC}{SLOC}
\newcommand{\Mtotal}{M}
\newcommand{\Mne}{M_{ne}}
\newcommand{\MnePro}{R_{ne}}
\newcommand{\Ttotal}{T}
\newcommand{\Tpm}{T_{d}}
\newcommand{\Tc}{T_c}
	


==> sections/evaluation.tex <==
\section{Research Questions}
\label{sec:evaluationdesign}


In this paper, we would like to investigate the following four research questions.


\noindent \textbf{RQ1:} \textbf{Are the refactored formulas functionally equal to original ones?} This question aims to check the correctness of our refactoring approach. To answer this question, we conduct manual inspection. Additionally, we replace the original formula with the refactored one in spreadsheets to check if they yield identical values. 

\noindent \textbf{RQ2:} \textbf{What is the refactor coverage of our approach?} This question aims to check the applicability of our approach: how many \nestifformu{} can our approach handle. We answer this question by presenting the total proportion of handled formulas as well as the number and proportion of formulas that each pattern handles.


\noindent \textbf{RQ3:} \textbf{What is the refactor effectiveness of our approach?} This question aims to check the \ifdepth{} reducing effectiveness of the refactoring. To answer this research question, we present the absolute number of reduced \ifdepth{} of each refactored formula, its proportion of reduced \ifdepth{}, as well as the final \ifdepth{} results of the refactored formulas. 
%We also present the spreadsheet file size comparison results before and after adopting the formula refactoring.

\noindent \textbf{RQ4:} \textbf{Do end users prefer the refactored formulas?} This question aims to find out the necessity of refactoring from the respective of end users, as well as whether end users prefer the refactored formula our approach provides. To do this, we survey end users with the original and refactored formulas and collect their opinions.


%\subsection{Experimental Process}
%To evaluate our approach, we choose the spreadsheet corpus introduced in our preliminary study~\ref{sec:premilinarystudy} out of its large scale, diversity, and new age as introduced previously. The evaluation process is described below.
%
%First, we scan each excel file in our corpus. We analyse each formula and extract\nestifformu{}. Among these formulas, we next remove some illegal formula if it is incomplete, or contains error messages\footnote{In excel, the error messages may include \emph{$\#DIV/0!$}, \emph{$\#N/A!$}, \emph{$\#NAME?$},\emph{$\#NULL!$}, \emph{$\#NUM!$}, \emph{$\#REF!$}, and \emph{$\#VALUE!$}.} The remaining formulas would be regarded as our analysis targets. 
%
%We next analyse the  \nestifformu{} one by one. Following the refactoring procedure introduced in Section~\ref{sec:approach}, we conduct automatic refactoring and get the new formula. Each newly refactored formula will be put back into the original position (to replace the old formula), so that we could check whether it would yield identical value as the old one (to answer RQ1).
%
%After finishing scanning all the excel files, we record the total set of original and refactored \nestifformu{} among all the files, and calculate the total refactor coverage (to answer RQ2). As introduced in Section~\ref{sec:premilinarystudy}, one spreadsheet may contain many similar formulas generated by dragging one formula down or right. To remove these kinds of similar formulas, we cluster all the formulas in one spreadsheet based on their R1C1 notation(see more in Section~\ref{sec:premilinarystudy}) and choose one formula from each cluster to compose the unique formula set, and calculate the unique refactor coverage (for RQ2). For each formula pair (original and refactored formula), we calculate the number as well as the proportion of reduced \ifdepth{} and formula length (for RQ3).
%
%Last, we do a survey on 49 people from various areas to investigate whether end users prefer using the refactored formulas.





